Understanding Social Media Cross-Modality Discourse in Linguistic Space

The multimedia communications with texts and images are popular on social media. However, limited studies concern how images are structured with texts to form coherent meanings in human cognition. To fill in the gap, we present a novel concept of cross-modality discourse, reflecting how human readers couple image and text understandings. Text descriptions are first derived from images (named as subtitles) in the multimedia contexts. Five labels -- entity-level insertion, projection and concretization and scene-level restatement and extension -- are further employed to shape the structure of subtitles and texts and present their joint meanings. As a pilot study, we also build the very first dataset containing 16K multimedia tweets with manually annotated discourse labels. The experimental results show that the multimedia encoder based on multi-head attention with captions is able to obtain the-state-of-the-art results.

==> figures/exp-attention.tex <==
\begin{figure*}[b]
\centering
\includegraphics[width=0.8\textwidth]{inputs/figure_attention.pdf}
\vspace{-0.5em}
\caption{Attention results}
\vspace{-0.5em}
\label{fig:att}
\end{figure*}

==> figures/exp-len.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=0.8\columnwidth]{inputs/figure_len_exp.pdf}
\caption{
F1 scores (y-axis) over varying text length to predict insertion, concretization, restatement, and extension discourse (x-axis). 
For each label, from left to right shows text input capped at 5, 10, 15, and 20. 
%test samples' word number in (0,5], (5,10], (10,15], and (15,20].
}
\label{fig:len_exp}
\end{figure}


==> figures/exp-similarity.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=0.6\columnwidth]{inputs/figure_similarity.pdf}
\vspace{-1em}
\caption{
Similarity scores (y-axis) over tweets labeled in insertion, concretization, restatement, and extension, from left to right. For each label, left bars in forward (blue) slash and right bars in back (green) slash show tweet texts' similarity with captions and subtitles.
}
\label{fig:simi}
\end{figure}


==> figures/intro-motivation.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=1.0\textwidth]{inputs/label_case.pdf}
\vspace{-2em}
\caption{Motivation for the task}
\vspace{-1em}
\label{fig:motivation}
\end{figure*}
